Word2Box: Capturing Set-Theoretic Semantics of Words using Box Embeddings

Learning representations of words in a continuous space is perhaps the most fundamental task in NLP, however words interact in ways much richer than vector dot product similarity can provide. Many relationships between words can be expressed set-theoretically, for example, adjective-noun compounds (eg. "red cars"$\subseteq$"cars") and homographs (eg. "tongue"$\cap$"body" should be similar to "mouth", while "tongue"$\cap$"language" should be similar to "dialect") have natural set-theoretic interpretations. Box embeddings are a novel region-based representation which provide the capability to perform these set-theoretic operations. In this work, we provide a fuzzy-set interpretation of box embeddings, and learn box representations of words using a set-theoretic training objective. We demonstrate improved performance on various word similarity tasks, particularly on less common words, and perform a quantitative and qualitative analysis exploring the additional unique expressivity provided by Word2Box.

==> sections/21_background_alternate.tex <==
\section{Background}
\label{sec:background}


\paragraph{Notations} Let $V=(v_i)_{i=1}^N$ denote the vocabulary in a fixed but arbitrary order, and $w=(v_i)_{i=1}^l$ be a sequence of words or a window of fixed length $l$. 
If $\mathcal W$ denotes the space of all windows of a fixed length $l$ and $I: \mathcal W \to \{0,1\}^{N}$ a function such that $I(w)_j = 1 \iff v_i\in w$, then since $I$ is bijection, we use $\mathcal W$ and $\{0,1\}^{N}$ interchangeably to denote the set of all windows. 
We use $\pi_j: \{0,1\}^{N} \to \{0,1\}, ~~j\in \{1, \dots, N\}$  to denote the canonical projection maps, i.e., we have $\pi_j(x) = x_j$.

\subsection{Fuzzy sets and distributional semantics}
\label{sec:fuzzy sets}

\dnp{We need a better, more generic example sentence in this paragraph.}
Given any ambient space $U$ a set $S\subseteq U$ can be represented by its characteristic function $\chi_S: U\to \{0, 1\}$ such that $\chi_S(u)=1 \iff u\in S$. This definition be generalized to $\bar \chi_S: U \to [0, 1]$ where $\bar\chi_S$ is the characteristic function of graded membership of a set $S$ which we now call a fuzzy set \citep{fuzzy-zadeh-1996}. 
Fuzzy sets are a useful way of thinking about language \cite{zhelezniak2018dont,note-on-fuzzy-language}. 
For instance, let $\mathcal W$, the set of all windows of a fixed length, be the ambient space, $w = \{\text{The, quick, brown, fox, jumped}\}\in \mathcal W$ be a window and $W_{\text{red}}$ denote the set of all windows that have center word \emph{red}.
It is easy to see that $\chi_{W_{\text{red}}}( \{\text{The, quick, brown, fox, jumped}\})=0$, because the center word $\text{brown}\not = \text{red}$. However, it is also clear that without more context, $w' = \{\text{The, quick, red, fox, jumped}\}$ is similar to $w$, and hence in a graded sense, $\chi_{W_{\text{red}}}( \{\text{The, quick, brown, fox, jumped}\})$ should be greater than $0$.
Similarly, let $\bar{W}_{\text{quick}}$ denote the set of all windows where \emph{quick} occurs as a non-center word, i.e., as a context word, then $\chi_{\bar{W}_{\text{quick}}}(\{\text{The, swift, brown, fox, jumped}\})$ should be greater than $0$ in the graded membership sense.
Hence, in order to capture the distributional semantics, we wish to learn a parametric model $M_{\Theta}: 2^{\mathcal W} \to (\mathcal W \to [0,1])$, i.e., a model that, given a set of windows, produces its graded membership function. \dnp{Here we might want to state, crisply if possible, what properties this model or the membership functions produces by it should have.} \dnp{If we write it this formally, one can think of several ways of constructing the model. Think about the "DON’T SETTLE FOR AVERAGE, GO FOR THE MAX:FUZZY SETS AND MAX-POOLED WORD VECTORS" paper. They also do something sensible. Here, we probably need more justification as why boxes!}
In the following section, we show how one can use box embeddings \cite{.} to construct such a model.

\subsection{Box embeddings}
\label{sec:box embeddings}

Now, in order to capture the distributional hypothesis \cite{something-old-and-fundamental,may-be-word2vec-and-glove} in a tractable manner, we are interested in modelling windows of the form $W_{v}$ and $\bar{W}_{v}$, where $v\in V$, using a parametric model. 
Let $F(\cdot~; \mu, \beta)$ and $G(\cdot~;\nu, \beta )$ denote the (cumulative) distribution functions of independent gumbel-max and gumbel-min random variables $X$ and $Y$ taking values in $\mathbb R$, where the distributions are  parameterized using the location parameters $\mu$ and $\nu$ and the temperature $\beta$.
Then 
\begin{align*}
P(X & < z < Y) =  F(x)[1-G(x)]\\
&=  \exp \left(-\exp(\frac{\mu-x}{\beta}) - \exp(\frac{x - \nu}{\beta})\right).
\end{align*}

We define a fuzzy set in $\mathbb R$ with membership function $\chi(z) = P(X < z < Y)$. 



If $\{X_k\}_{k=1}^d$ and  $\{Y_k\}_{k=1}^d$ are collections of independent random variables with gumbel-max ($\{F_k (\cdot~; \mu, \beta)\}_{k=1}^d$) and gumbel-min ($\{G_k(\cdot~; \nu, \beta)\}_{k=1}^d$) distributions, respectively, where $\mu, \nu$ are the location parameters and $\beta$ is the temperature parameter.
Then the probability of point $x\in \mathbb R^d$ to be inside $\BoxE(X,Y)$, denoted as $\chi_{\BoxE(X,Y)}(x)$ is given as
\begin{align*}
\chi(x) &= \prod_{k=1}^d F_{k}(x)[1-G_{k}(x)]\\
\log \chi(x) &=  \sum_{k=1}^d -\exp(\frac{\mu-x}{\beta}) - \exp(\frac{x - \nu}{\beta}).
\end{align*}


\dnp{Here we are going through rectangles whose endpoints are gumbel random variables, which after writing it out, seems a little convoluted. Would it be better if we used the observation made in the UAI paper that these are densities of the form $(1-F_{Y}(z))F_X(z)$ and start from there?}
%If each window $w\in \{0,1\}^N$ is represented as a point $f(w) \in \mathbb R^d$, then the set of windows $W_{v}$ is a collection of points $f(W_v)\subseteq R^d$, where $v\in V$ is word in the vocabulary. 


%Moreover, as discussed in section \ref{sec:fuzzy sets}, we want $B^{-1}(W)$ to be a fuzzy set in $\mathbb R^d$.
Let $B:  \mathbb R^d \to \{0,1\}^{N}$ be some function that maps points in $\mathbb R^d$ to  windows of fixed length.
Then if $W\in 2^{\{0,1\}^N}$ is some set of windows, we have that $B^{-1}(W) \subseteq \mathbb R^d$.
Moreover, the inverse map $B^{-1}(W)$ can be used to induce a membership function using the indicator function $\mathbf{1}_{B^{-1}(W)}: \mathbb R \to [0,1]$ on points in $\mathbb R^d$, which intern produces the membership function $\mathbf{1}_{W}: \mathcal W \to [0,1]$ where $\mathbf{1}_{W}(w) = \mathbf{1}_{B^{-1}(W)} (B^{-1}(w))$.
\dnp{Between here and the next paragraph, I see a lot of design choices. We will need to justify why we restrict the map $B$ to be such that it is a box.}

Now, in order to capture the distributional hypothesis \cite{something-old-and-fundamental,may-be-word2vec-and-glove} in a tractable manner, we are interested in modelling windows of the form $W_{v}$ and $\bar{W}_{v}$, where $v\in V$, using a parametric model.
We get one such model if restrict $B$ to be such that $B^{-1}(W_{v}) = \prod_{k=1}^d [x^v_{k}, y^v_{k}] := \BoxE(x^v, y^v)$ where $x^v, y^v \in \mathbb R^d$ are free parameters with the restriction that $x^v_{k} \leq y^v_{k}$. Similarly, we restrict $B^{-1}(\bar{W}_w)$ to be $\BoxE(\bar{x}^v, \bar{y}^v)$.
\dnp{This is a bit sloppy. It can be made better later.}
\dnp{I can reduce the math jargon later but I want to keep it for now for my understanding.}
\dnp{Here we will say that instead of using an indicator function, we will use something soft to make the membership function graded. Again, here I see a lot of choices, and we will need to justify why we should use gumbel. Yes it results in closure under intersection but if it is equivalent to product T-norm, why not just use some other soft membership and use T-norm on that?}

\points{
DP: Next I will add the formula for membership of a point in a gumbel box and state that a gumbel box defines a fuzzy set in $\mathbb R^d$ by showing the equivalence with product T-norm.
}

As noted in \citet{boratko2021min}, when the min (resp. max) coordinates of the box are taken to be gumbel-max (resp. gumbel-min) random variables, then the probability of a point being inside can be computed easily.\dnp{The end it a bit vague. Need to remove 'easlily' and say something concrete.}
If $\{X_k\}_{k=1}^d$ and  $\{Y_k\}_{k=1}^d$ are collections of independent random variables with gumbel-max ($\{F_k (\cdot~; \mu, \beta)\}_{k=1}^d$) and gumbel-min ($\{G_k(\cdot~; \nu, \beta)\}_{k=1}^d$) distributions, respectively, where $\mu, \nu$ are the location parameters and $\beta$ is the temperature parameter.
Then the probability of point $x\in \mathbb R^d$ to be inside $\BoxE(X,Y)$, denoted as $\chi_{\BoxE(X,Y)}(x)$ is given as
\begin{align*}
\chi(x) &= \prod_{k=1}^d F_{k}(x)[1-G_{k}(x)]\\
\log \chi(x) &=  \sum_{k=1}^d -\exp(\frac{\mu-x}{\beta}) - \exp(\frac{x - \nu}{\beta}).
\end{align*}
It is interesting to note the following properties of the fuzzy sets defined using boxes (proofs are given in the appendix)\dnp{May be copy paste what Michael wrote on notion?}.
\remark{$\chi$ is the membership function of a fuzzy set in $\mathbb R^d$}
\remark{The box intersection as defined in \cite{Dasgupta2020ImprovingEmbeddings} is actually the intersection of corresponding fuzzy sets under the product T-norm.}  


==> tables/all_operations_bank_finance.tex <==
\resizebox{\linewidth}{!}{%
    \centering
\begin{tabular}{|lll|llllll|}
\hline
\multicolumn{3}{|c|}{\wb} & \multicolumn{6}{c|}{\wv}\\ \hline
\multicolumn{1}{|l|}{bank $\cap$ finance} & \multicolumn{1}{l|}{bank $\cup$ finance} & bank $\setminus$ finance & \multicolumn{1}{l|}{bank + finance} & \multicolumn{1}{l|}{bank - finance} & \multicolumn{1}{l|}{max(bank, finance)} & \multicolumn{1}{l|}{min(bank, finance)} & \multicolumn{1}{l|}{max\_score(bank, finance)} & min\_score(bank, finance) \\ \hline
investment                           & banking                             & wensum                            & subprime                            & shaddai                             & subprime                                & liquidity                               & refinance                                      & securities                \\
banking                              & treasury                            & junction                          & securities                          & takla                               & securities                              & refinance                               & laundering                                     & subprime                  \\
investor                             & investor                            & neman                             & refinance                           & thrombus                            & underwrite                              & kaupthing                               & reimbursements                                 & jpmorgan                  \\
financing                            & investment                          & mouth                             & liquidity                           & gauley                              & interlibrary                            & cibc                                    & superannuation                                 & citigroup                 \\
fund                                 & business                            & tributary                         & laundering                          & paria                               & refinance                               & securities                              & liquidity                                      & equities                  \\
government                           & economy                             & downstream                        & kaupthing                           & epenthetic                          & codeshare                               & cellulosic                              & debit                                          & ebrd                      \\
corporation                          & management                          & corner                            & underwrite                          & chibchan                            & brokerage                               & bbdo                                    & controllata                                    & kaupthing                 \\
treasury                             & firm                                & embankment                        & receivables                         & urubamba                            & borrower                                & berhad                                  & subprime                                       & mortgage                  \\
citigroup                            & fund                                & forks                             & ibrd                                & foremast                            & jpmorgan                                & automakers                              & underwrite                                     & refinance                 \\
firm                                 & financial                           & sandwich                          & equities                            & bolshaya                            & laundering                              & reits                                   & disbursement                                   & debentures \\
\hline
\end{tabular}
}

==> tables/single_column.tex <==
\begin{table}[!htbp]
\resizebox{\linewidth}{!}{%
    \centering
    \begin{table}[]
\begin{tabular}{|lll|llllll|}
\hline
\multicolumn{3}{|l|}{\wb}                                                                       & \multicolumn{6}{l|}{\wv}                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{bank $\cap$ finance} & \multicolumn{1}{l|}{bank $\cup$ finance} & bank $\setminus$ finance & \multicolumn{1}{l|}{bank + finance} & \multicolumn{1}{l|}{bank - finance} & \multicolumn{1}{l|}{max(bank, finance)} & \multicolumn{1}{l|}{min(bank, finance)} & \multicolumn{1}{l|}{max\_score(bank, finance)} & min\_score(bank, finance) \\ \hline
investment                           & banking                             & wensum                            & subprime                            & shaddai                             & subprime                                & liquidity                               & refinance                                      & securities                \\
banking                              & treasury                            & junction                          & securities                          & takla                               & securities                              & refinance                               & laundering                                     & subprime                  \\
investor                             & investor                            & neman                             & refinance                           & thrombus                            & underwrite                              & kaupthing                               & reimbursements                                 & jpmorgan                  \\
financing                            & investment                          & mouth                             & liquidity                           & gauley                              & interlibrary                            & cibc                                    & superannuation                                 & citigroup                 \\
fund                                 & business                            & tributary                         & laundering                          & paria                               & refinance                               & securities                              & liquidity                                      & equities                  \\
government                           & economy                             & downstream                        & kaupthing                           & epenthetic                          & codeshare                               & cellulosic                              & debit                                          & ebrd                      \\
corporation                          & management                          & corner                            & underwrite                          & chibchan                            & brokerage                               & bbdo                                    & controllata                                    & kaupthing                 \\
treasury                             & firm                                & embankment                        & receivables                         & urubamba                            & borrower                                & berhad                                  & subprime                                       & mortgage                  \\
citigroup                            & fund                                & forks                             & ibrd                                & foremast                            & jpmorgan                                & automakers                              & underwrite                                     & refinance                 \\
firm                                 & financial                           & sandwich                          & equities                            & bolshaya                            & laundering                              & reits                                   & disbursement                                   & debentures               
\end{tabular}
\end{table}
    }
    \caption{Output of \wb and \wv for various set-operations}
    \label{table:set_operations_comparison}
\end{table}


% \begin{table*}[htbp]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llp{0.8\linewidth}}
% \toprule
%      &     &                                         Similarity \\
% Word & Model &                                                    \\
% \midrule
% bank &  \wb &  capital settlement airline hotel gateway treas... \\
%      & \textbackslash wv &  debit depositors securities kaupthing interban... \\
% economics & \textbackslash wb &  education architecture politics economy litera... \\
%      & \textbackslash wv &  microeconomic keynesian microeconomics minored... \\
% microeconomics & \textbackslash wb &  economics mathematics physics philosophy theor... \\
%      & \textbackslash wv &  microeconomic initio germline instantiation za... \\
% property & \textbackslash wb &  land register status manor purpose locality pr... \\
%      & \textbackslash wv &  easement infringes burgage krajobrazowy chatte... \\
% rock & \textbackslash wb &           music pop mountain cave band blues dance \\
%      & \textbackslash wv &  shoegaze rhyolitic punk britpop mafic outcrops... \\
% \bottomrule
% \end{tabular}
% \caption{Similarity outputs for \wb and \wv}
% \label{table:similarity}
% \end{table*}
\begin{table*}[htbp]
\begin{tabular}{lll}
\toprule
{} &                                                     \wb \\ $A \cap X$ &                                                                                                              \wv \\ $A \cdot X$ \\
A              &                                                                       &                                                                                                                                 \\
\midrule
bank           &                capital settlement airline hotel gateway treasury firm &                                      debit depositors securities kaupthing interbank subprime counterparty citibank fdic nasdaq \\
economics      &            education architecture politics economy literature faculty &  microeconomic keynesian microeconomics minored macroeconomics econometrics sociology thermodynamics evolutionism structuralist \\
microeconomics &  economics mathematics physics philosophy theory technology economist &                  microeconomic initio germline instantiation zachman macroeconomics oxoglutarate glycemic noncommutative pubmed \\
property       &                   land register status manor purpose locality premise &                           easement infringes burgage krajobrazowy chattels policyholder leasehold intestate liabilities ceteris \\
rock           &                              music pop mountain cave band blues dance &                                           shoegaze rhyolitic punk britpop mafic outcrops metalcore bluesy sedimentary quartzite \\
\bottomrule
\end{tabular}
\caption{Similarity outputs for \wb and \wv}
\label{table:similarity}
\end{table*}

\begin{table*}
\centering
\resizebox{0.98\linewidth}{!}{%
\begin{tabular}{llllp{0.6\linewidth}}
\toprule
       &          &                                                                   \wb \\ $(A \cap B) \cap X$ &                                                                      \wv \\ $(A + B) \cdot X$ \\
A & B &                                                                                              &                                                                                               \\
\midrule
girl & boy &                           kid girls schoolgirl teenager woman boys child baby teenage orphan &                    shoeshine nanoha soulja schoolgirl yeller beastie jeezy crudup 'girl rahne \\
property & burial &                cemetery bury estate grave interment tomb dwelling site gravesite sarcophagus &        interment moated interred dunams ceteris burials catafalque easement deeded inhumation \\
       & historical &  historic estate artifact archaeological preserve ownership patrimony heritage landmark site &  krajobrazowy burgage easement kravis dilapidation tohono intangible domesday moated laertius \\
       & house &               estate mansion manor residence houses tenement building premise buildings site &       leasehold mansion tenements outbuildings estate burgage bedrooms moated burgesses manor \\
tongue & body &                                       eye mouth ear limb lip forehead anus neck finger penis &      tubercle ribcage meatus diverticulum forelegs radula tuberosity elastin foramen nostrils \\
       & language &            dialect idiom pronunciation meaning cognate word accent colloquial speaking speak &         fluently dialects vowels patois languages loanwords phonology lingala tigrinya fluent \\
\bottomrule
\end{tabular}
}
\caption{Comparison of set intersection operation}
\label{table:intersection}
\end{table*}

\begin{table*}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{llllp{0.6\linewidth}}
\toprule
         &      &                                                                               \wb \\ $(A \setminus B) \cap X$ &                                                                                                   \wv \\ $(A - B) \cdot X$ \\
A & B &                                                                                                               &                                                                                                                            \\
\midrule
algebra & finance &    homomorphism isomorphism automorphism abelian algebraic bilinear topological morphism spinor homeomorphism &  homeomorphic unital homomorphisms nilpotent algebraically projective holomorphic propositional nondegenerate endomorphism \\
bank & finance &                             wensum junction neman mouth tributary downstream corner embankment forks sandwich &                                         shaddai takla thrombus gauley paria epenthetic chibchan urubamba foremast bolshaya \\
         & river &                                    barclays hsbc banking citigroup citibank firm ipo brokerage interbank kpmg &                            cheques tymoshenko receivables citibank eurozone brinks defrauded courtaulds refinance mortgage \\
chemistry & finance &            biochemistry superconductor physics physic eutectic heat isotope fluorescence yttrium spectroscopy &                  augite alkyne desorption phosphorylating dimorphism fumarate hypertrophic empedocles hydratase enantiomer \\
property & land &  homotopy isomorphism involution register bijection symplectic eigenvalue idempotent compactification lattice &                                                brst stieltjes l'p repressor absurdum doesn conjugates nonempty didn wouldn \\
\bottomrule
\end{tabular}
}
\caption{Comparison of set difference operation}
\label{table:set_difference}
\end{table*}
\begin{table*}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllllp{0.6\linewidth}}
\toprule
         &         &           &                                                                   \wb \\ $(A \setminus B) \cap C) \cap X$ &                                                                          \wv \\ $(A - B + C) \cdot X$ \\
A & B & C &                                                                                                           &                                                                                                       \\
\midrule
property & finance & algebra &  laplacian nilpotent antiderivative lattice surjective automorphism invertible homotopy integer integrand &    expropriate extort refco underwrite reimburse refinance parmalat refinancing brokerage privatizing \\
         &         & chemistry &    eutectic desiccant allotrope phenocryst hardness solubility monoclinic hygroscopic nepheline trehalose &  refinance brokerage burgage stockbroking refinancing warranties reimburse madoff privatizing valorem \\
\bottomrule
\end{tabular}
}
\caption{Comparison of set difference followed by intersection operation}
\label{table:set_difference_intersection}
\end{table*}
